CAPTURE: Minimizing Watch Time for Reliable Temporal Video Grounding

Video grounding models typically answer a text query with a single time span, without guaranteeing that it matches the requested moment. We ask how little of the video a person must watch to find a matching clip with a prescribed probability. Prior conformal grounding can widen an answer to contain the whole moment, although a viewer only needs footage containing one clip at the required temporal intersection-over-union (tIoU). We introduce CAPTURE, which uses a frozen grounder's probabilities over candidate spans to find short footage that contains such a clip. For tIoU of at least 0.5, its exact dynamic program guarantees minimum possible watch time at a given model coverage level. Conformal calibration on held-out examples then determines how much footage to return to meet the requested success rate. We establish marginal coverage and a high-probability watch-duration bound relative to an oracle with access to the true conditional distribution. A matching lower bound shows that the dependence on grounding-model errors is unavoidable in the worst case. Efficient heuristics retain the coverage guarantee when scoring all spans is impractical. Experiments on Charades-STA, QVHighlights and ActivityNet Captions show that CAPTURE, across six grounding backbones, achieves the prescribed tIoU coverage while reducing average watch duration by approximately 35% compared with prior methods. We release our code at https://github.com/aliasgerovs/capture.

==> fig/dp.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\textwidth]{fig/dp-figure.pdf}
\caption{\textbf{The dynamic program finds the shortest watched region whose model-estimated success probability reaches $q_0$.}
This toy example applies \cref{alg:watch} to a 6-second video with $\tau=0.7$ and $q_0=0.75$.
(a)~A segment's value $c(a,b)$ sums the probabilities of candidate moments whose overlap with the segment is at least $\tau$ times the moment's length.
(b)~Entry $F_t(w)$ is the largest model-estimated success probability attainable inside $[0,t]$ with at most $w$ seconds watched. The recurrence takes the larger value obtained by leaving second $t$ unwatched or by ending a segment there.
(c)~The final row first reaches $q_0$ at $w=3$. Tracing the saved choices backward returns the segments $[1,3]$ and $[4,5]$.}
\label{fig:supp:dp}
\end{figure*}


==> fig/watch-distribution.tex <==
\begin{figure}[b]
\centering
\includegraphics[width=\linewidth]{fig/watch-distribution-figure.pdf}
\caption{\textbf{\texttt{CAPTURE} adapts watch duration to each query.}
The figure shows Qwen3-VL-8B on the 654 test queries of one QVHighlights split, with tIoU threshold 0.5 and 80\% requested success rate.
Watch duration is normalized by video length.
The dashed line marks the median normalized watch duration.}
\label{fig:watch-distribution}\hypertarget{figure.caption.21}{}%
\end{figure}


==> sec/2_related.tex <==
\section{Extended related work}
\label{sec:related}

\paragraph{Conformal prediction and risk control.}
Split-conformal prediction calibrates a prediction set on held-out labeled examples, with marginal coverage under exchangeability~\cite{vovk2005algorithmic,papadopoulos2002inductive,lei2018distribution}.
Hierarchical methods allow examples within a group to be dependent~\cite{dunn2018hierarchical,lee2023hierarchical}.
Risk-control methods instead bound average loss~\cite{bates2021rcps,angelopoulos2024crc}.
We treat videos as independent units and draw one query uniformly from each, so the guarantee concerns a query drawn the same way from a new video and allows related errors within a video.

\paragraph{Sets of generated answers.}
Conformal language modeling~\cite{quach2024clm} and TRON for video questions~\cite{wang2025tron} calibrate sets of sampled answers.
Other methods filter unreliable claims~\cite{mohri2024factuality} or use repeated answers without model probabilities~\cite{su2024api,wang2024conu}.
Our finite temporal grid permits scoring all candidate spans.
We use their probabilities to construct the region and matching-clip success on calibration examples to decide how much footage to return.
This extends minimum Bayes risk decoding from one answer to a set of spans, counting overlapping footage once~\cite{kumar2004mbr,ichihara2025mbr}.

\paragraph{Containment and watch duration.}
Conformal detection and segmentation enlarge regions to contain objects~\cite{timans2024twostep,andeol2023railway,davenport2024segmentation,mossina2024conformal}.
Lu et al.~\cite{lu2026instance} instead calibrate sets of instance masks in which at least one reaches a requested IoU, a target closer to ours.
Prior conformal temporal grounding, COVER~\cite{mohamed2026cover}, similarly widens an interval or forms a relevance level set and studies its size.
Containing a whole moment supplies a clip at any tIoU but can require more viewing than one matching clip.
\Cref{sec:supp:results:fair} isolates this distinction from the benefit of region construction.

\paragraph{Notes on technical novelty.}
Our work builds on the connection between conformal prediction and volume-optimal prediction sets studied by Gao et al.~\cite{gao2025volume}, but introduces distinct statistical and computational challenges.
Unlike their regression setting, where coverage is determined by set membership, our coverage criterion requires at least one predicted span, or a clip within the watched region, to achieve sufficient tIoU, while watch duration measures the union of selected intervals.
This distinction leads to a different optimization problem, in which coverage depends on the existence of a sufficiently accurate subinterval within the selected footage, while viewing cost depends on the total duration of that footage.
A key technical challenge is ensuring that conformal calibration preserves the duration efficiency of the model-optimal solution.
We address this through an inclusion-minimal anchor that connects the calibrated prediction to its watch-duration bound.
Our analysis further exploits marginal coverage to require only average control of model overestimation, while controlling underestimation on most inputs to obtain conditional-oracle comparisons, unlike the more restrictive two-sided high-probability accuracy conditions of Gao et al.~\cite{gao2025volume}.
Finally, a matching minimax lower bound establishes the asymptotic sharpness of the coverage relaxation in our oracle comparison.


==> sec/7_llm.tex <==
\paragraph{LLM usage statement.}
We used Claude (Anthropic) and ChatGPT (OpenAI).
For code and implementation and for figures, the tools generated parts of the work, which the authors reviewed, edited and approved.
For figures, this was the code that draws them, such as \cref{fig:method}.
For writing, related work and citations, experiments, and research ideas and conclusions, the tools only assisted by editing or refining content produced by the authors.
No tool was used for data creation or annotation.
The authors designed the study, chose and approved the experiments, verified the code and outputs, checked the citations and reported values, and remain responsible for all scientific claims and submitted content.


==> sec/S_set.tex <==
\appendix
\makeatletter\global\advance\Hy@linkcounter by 1000\relax\makeatother
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{equation}{0}
\renewcommand{\thefigure}{S\number\numexpr\value{figure}\ifnum\value{figure}>2 +1\fi\relax}
\renewcommand{\thetable}{S\arabic{table}}
\renewcommand{\theequation}{S\arabic{equation}}
\renewcommand{\theHfigure}{\thefigure}
\renewcommand{\theHtable}{S\arabic{table}}
\renewcommand{\theHequation}{S\arabic{equation}}
\renewcommand{\thealgorithm}{S\arabic{algorithm}}
\providecommand{\theHalgorithm}{}\renewcommand{\theHalgorithm}{S\arabic{algorithm}}
\makeatletter
\let\supp@input\input
\newcommand{\supppinnedfig}[2]{\begingroup\edef\supp@savedfig{\number\value{figure}}\setcounter{figure}{\numexpr#2-1\relax}\renewcommand{\thefigure}{S\arabic{figure}}\renewcommand{\theHfigure}{S\arabic{figure}}\supp@input{#1}\setcounter{figure}{\supp@savedfig}\endgroup}
\expandafter\def\csname supp@pin@set_methods_full\endcsname{1}
\expandafter\def\csname supp@pin@set_watch\endcsname{2}
\expandafter\def\csname supp@pin@set_quality\endcsname{3}
\expandafter\def\csname supp@pin@set_chlong\endcsname{9}
\expandafter\def\csname supp@pin@set_newpools\endcsname{11}
\expandafter\def\csname supp@pin@set_size\endcsname{12}
\expandafter\def\csname supp@pin@set_calsize\endcsname{33}
\expandafter\def\csname supp@pin@set_runtime\endcsname{4}
\expandafter\def\csname supp@pin@set_tau1\endcsname{5}
\expandafter\def\csname supp@pin@set_structure\endcsname{7}
\expandafter\def\csname supp@pin@set_retarget\endcsname{10}
\expandafter\def\csname supp@pin@set_units\endcsname{13}
\expandafter\def\csname supp@pin@set_q0\endcsname{14}
\expandafter\def\csname supp@pin@set_strata\endcsname{15}
\expandafter\def\csname supp@pin@set_equal\endcsname{16}
\expandafter\def\csname supp@pin@set_delta\endcsname{17}
\expandafter\def\csname supp@pin@set_fact\endcsname{18}
\expandafter\def\csname supp@pin@set_mbr\endcsname{19}
\expandafter\def\csname supp@pin@set_cap\endcsname{21}
\newcommand{\supptab}[1]{%
\par
\@ifundefined{supp@tab@#1}{\expandafter\gdef\csname supp@tab@#1\endcsname{}%
\@ifundefined{supp@pin@#1}{\PackageError{supp}{No fixed number for table #1}{}}{\setcounter{table}{\numexpr\csname supp@pin@#1\endcsname-1\relax}}%
\supp@input{tables/supp/#1}}{}%
\par}
\@ifundefined{suppresult}{%
\newenvironment{suppresult}[1]%
{\par\addvspace{\medskipamount}\noindent\textbf{#1.}\ \itshape\ignorespaces}%
{\par\addvspace{\medskipamount}}%
}{}
\makeatother

\noindent This supplement gives the proofs, implementation details and full evaluations of \texttt{CAPTURE}. Its main points are:
\begin{itemize}
\item \textbf{Most of the saving over prior methods comes from the matching-clip guarantee.} When both methods must contain the whole moment, the saving at an 80\% requested success rate falls from 28\% of the video at tIoU 0.5 to 2\%. COVER recalibrated for one matching clip still watches 48.2\% of the video on average, against 43.1\% for \texttt{CAPTURE}, which watches less in 86 of 108 cells (\cref{sec:supp:results:fair}).
\item \textbf{Calibrating on videos attains the requested success rate.} With one query per calibration video, mean success is never more than about 0.001 below the request, while calibrating on all queries falls more than 0.002 short in 22 of 72 cells. One tenth of the calibration videos still meets the requested rate, with up to 11\% more of the video watched (\cref{sec:supp:results:calibration}).
\item \textbf{Cheaper anchors keep the guarantee but watch more.} With equal labeled-video budgets, the greedy and MBR anchors watch 49.0\% and 46.0\% of the video on average and COVER 65.1\%, against 42.7\%--43.5\% for the span-based regions (\cref{sec:supp:results:regions}).
\item \textbf{The sufficient watch-duration condition is conservative.} Anchors succeed less often than their threshold predicts in all 72 settings, so the condition does not certify short regions for today's grounders, while marginal coverage still holds. The matching lower bound shows that the dependence on grounding-model errors is unavoidable in the worst case (\cref{sec:supp:results:bound,sec:supp:proofs:lower}).
\item \textbf{Less watch duration across model sizes.} Across seven models from 2B to 32B, it watches less than COVER in all 126 cells and less than the greedy anchor in 120 (\cref{sec:supp:results:generalization}).
\item \textbf{Efficient heuristics retain the coverage guarantee.} Scoring all spans takes 0.7 to 5.6 times as long as greedy decoding; on QVHighlights, about 6.5 more GPU seconds per query save about 55 seconds of viewing per 150-second video against COVER. When scoring all spans is impractical, two-prompt scoring with a learned correction removes 86\% and 93\% of its extra watch duration on QVHighlights and ActivityNet Captions (\cref{sec:supp:results:distribution,sec:supp:impl:factorized}).
\item \textbf{Coverage is marginal.} It is not guaranteed separately by moment length or video duration: success ranges from 73\% to 91\% across moment lengths at tIoU 0.5 and 80\%. Viewers must still find the matching clip within the selected footage, and a second model pass on it need not succeed (\cref{sec:supp:results:regions}).
\end{itemize}

\paragraph{Reported configurations.}
\texttt{CAPTURE} in the main paper uses the exact anchor, followed by the remaining spans in decreasing model probability; tables label it \emph{exact anchor (main paper)}.
As an ablation, we also report a variant that selects the region type together with $q_0$ on the fit videos (\cref{sec:supp:impl:regions}), labeled \emph{region type selected on fit videos}.
It appears only in \cref{tab:supp:quality,tab:supp:newpools,tab:supp:size,tab:supp:units}, which do not report the main-paper configuration, and in the qualitative examples of \cref{fig:supp:qualitative-success,fig:supp:qualitative-failure}.
Across the 108 cells of \cref{tab:main}, its normalized watch duration differs from the main-paper configuration by 0.018 on average and by at most 0.075.
Both use independent calibration videos and the same matching-clip success rule.

\setcounter{tocdepth}{2}
\begingroup
\small
\tableofcontents
\endgroup
\newpage

\input{sec/supp/proofs}
\FloatBarrier
\input{sec/supp/implementation}
\FloatBarrier
\input{sec/supp/results}
\input{sec/2_related}
\FloatBarrier

\input{sec/7_llm}

